Investigating Psychological Ownership in a Shared AR Space: Effects of Human and Object Reality and Object Controllability

Augmented reality (AR) provides users with a unique social space where virtual objects are natural parts of the real world. The users can interact with 3D virtual objects and virtual humans projected onto the physical environment. This work examines perceived ownership based on the reality of objects and partners, as well as object controllability in a shared AR setting. Our formal user study with 28 participants shows a sense of possession, control, separation, and partner presence affect their perceived ownership of a shared object. Finally, we discuss the findings and present a conclusion.

==> Contents/old/4_evaluation.tex <==
\section{Evaluation}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Contents/Figure/regression_result_placeholder.png}
    \caption{placeholder, 1. add sense of bond 2. unify the terms
    }
    \label{fig_regression_result}
\end{figure*}


\subsection{Participants}
We recruited 28 participants via SONA. They include 15 males and 15 females with an average age of 20.0 years (from 18 to 24). All participants have (corrected) 20/20 vision. 
% 19 participants reported they have experience using AR applications, and their self-familiarity score with AR is an average of x out of 7.0. %All the participants received 0.5 SONA credits as a reward. 
The study takes approximately 30 minutes, and the participants are given 1.5 SONA credits as a reward. The 1.5 SONA credits are the maximum reward for a 30-minute in-person study in accordance with IRB regulations. Our study is approved by IRB (IRB \#13233).


\subsection{Hypothesis}

Our hypotheses are as follows.

\begin{enumerate}
[label=H\arabic*., noitemsep]
\item The participant will have a stronger sense of ownership factors when the tangibility of a shared object is real rather than virtual. 
\item The participant's ownership factors of the shared object will be hampered when the tangibility of the partner is a real human rather than a virtual human. 
\item Having control over an object will reinforce the perceived ownership factors of the object.
\end{enumerate}



% \paragraph{Big Five Personality Traits:}

\subsection{Analysis}

Statistical analyses including within-subject 4-way repeated ANOVA and logistic regression analysis are  performed to analyze the measurements. %In the following section, 
\HDY{The four independent variables are object presence (OP), partner presence (PP), participant's controllability (PTC), and partner's controllability (PNC).}
We first report the ANOVA results regarding the four ownership and two presence factors. 
%The ANOVA test is corrected with Bonferroni correction. The degrees of freedom are also corrected using the Greenhouse-Geisser correction to avoid the sphericity assumption violations. 
The Bonferroni pairwise comparison test is used as a posthoc test when ANOVA shows a significant effect. Next, logistic regression results are reported to examine the effect of the factors on user-perceived ownership of the objects. We use scikit-learn~\cite{scikit-learn}, a Python package, to fit a logistics regression model. The significance level for all tests is set at 5\%.

\subsection{Results}
% \ic{I think it maybe better to have a table.}
Table~\ref{result_table} shows all significant main and interaction effects of the experimental factors. 

\bgroup
\def\arraystretch{1.2}%
\begin{table}[t]
\centering
\normalsize
\caption{\label{result_table} \textbf{...}}
% \begin{tabular}{l|l|l|l|l|l}
% \begin{tabular} {m{3cm} | m{2.5cm} | m{1cm} | m{1cm}| m{1cm} | m{0.8cm}}
\begin{tabular} {m{2cm} | m{1.5cm} | m{1cm} | m{0.9cm}| m{0.7cm}}
% \cline{1-6}
\toprule
\textbf{Measurement} & \textbf{Factor}  &  {\textbf{$F(1, 27)$}} & {\textbf{$p$}} & {\textbf{$\eta$\textsubscript{$p$}\textsuperscript{$2$}}}\\
\midrule
\cellcolor[gray]{0.9}    & {PTC \texttimes{} PNC}     &  {14.0} & {\textless.001}  &  {.342}  \\ \cline{2-5}
\cellcolor[gray]{0.9}   \textbf{Sense of}   & {OP}   &   {15.7}  & {\textless.001}  & {.369}    \\ \cline{2-5}
\cellcolor[gray]{0.9}   \textbf{Belongings}  &  {PTC}      &  {108}  & {\textless.001}  & {.800}   \\ \cline{2-5}
\cellcolor[gray]{0.9}   &  {PNC}      &  {10.5}  & {.003}  & {.280}   \\
% \cline{1-6}
\midrule
% \textbf{Difference} \newline (Q1 - Non-Missing Avg) vs. (Q1 - Avg)  & {MD}     &  {3, 150}   &  {1.68} & {.188}  &  {.032}  \\ 
                    & {PTC \texttimes{} PNC}      &  {7.38}  &  {.011} &  {.215}  \\ \cline{2-5}
\textbf{Sense of}   & {OP}      &  {4.61} &  {.041} &   {.146} \\ \cline{2-5}
\textbf{Control}    & {PTC}      & 244  & \textless .001  &  .900 \\ \cline{2-5}
                    & {PNC}    &  8.14  & .008  &  .232  \\ 
\midrule
\cellcolor[gray]{0.9}                       & {PTC \texttimes{} PNC}      &  {18.1} &  {\textless.001} &  {.401}  \\ \cline{2-5}
\cellcolor[gray]{0.9}  \textbf{Sense of}    & {OP}      &   {8.08}  & {.008}  & {.230}   \\ \cline{2-5}
\cellcolor[gray]{0.9}  \textbf{Bond}        & {PTC}      &  {124} & {\textless.001}  &  {.821}  \\\cline{2-5}
\cellcolor[gray]{0.9}                       & {PNC}      &  {6.02} & {.021}  &  {.182}  \\
\midrule
% \textbf{Difference} \newline (Q1 - Non-Missing Avg) vs. (Q1 - Avg)  & {MD}     &  {3, 150}   &  {1.68} & {.188}  &  {.032}  \\ 
\textbf{Sense of}   & {OP \texttimes{} PNC}      &  {13.7}  &  {\textless.001} &  {.337}  \\ \cline{2-5}
\textbf{Separation} & {OP}      &  {4.88} &  {.036} &   {.153} \\ \cline{2-5}
                    & {PTC}      &  {32.1}  & \textless .001  &  {.543}  \\ 
\midrule

\cellcolor[gray]{0.9} \textbf{Sense of}    & {OP \texttimes{} PP}    & {5.28} &  {.030} &  {.163}  \\ \cline{2-5}
\cellcolor[gray]{0.9} \textbf{Coexistance} & {OP \texttimes{} PTC}   &  {5.45} &  {.027} &  {.168}  \\ \cline{2-5}
\cellcolor[gray]{0.9} \textbf{(Object)} & {OP}      &   {76.9}  & {\textless.001}  & {.740}   \\ \cline{2-5}
 \cellcolor[gray]{0.9}                  & {PTC}      &  {28.4} & {\textless.001}  &  {.512}  \\
\midrule
% \textbf{Difference} \newline (Q1 - Non-Missing Avg) vs. (Q1 - Avg)  & {MD}     &  {3, 150}   &  {1.68} & {.188}  &  {.032}  \\ 
\textbf{Sense of}   & {PTC \texttimes{}PNC}      &  {4.34}  &  {.047} &  {.139}  \\ \cline{2-5}
\textbf{Coexistance}  & {PP}      &  {84.6} &  {\textless.001} &   {.758} \\ \cline{2-5}
\textbf{(Partner)}  & {PNC}      &  {6.59}  & {.016}  &  {.196}  \\ 
\bottomrule
\end{tabular}

\end{table}

\subsubsection{ANOVA Results on Ownership Factors and Presence}



\textbf{Sense of belonging}:
PNC and PRC show a significant interaction effect ($p\textless.001$). 
% PNC and PRC show a significant interaction effect ($p\textless.001$,  $F(1, 27)=14.0$, ${\eta_p}^2=.342$). 
Following that, a simple effect of PNC is revealed when the participants have object controllability ($p\textless.001$).%,  $F(1, 27)=31.9$, ${\eta_p}^2=.542$). 
Between the cases when the partner has no control over the object and when they do, the former ($M=5.54$) has a statistically greater sense of belonging than the latter ($M=4.69$).


% The main effects of OP ($p\textless.001$, $F(1, 27)=15.7$, $eta_p2=.369$), PTC ($p\textless.001$, $F(1, 27)=108$, $eta_p2=.800$), and PNC ($p=.003$, $F(1, 27)=10.5$, $eta_p2=.280$) are also found. 
The main effects of OP ($p\textless.001$), PTC ($p\textless.001$), and PNC ($p=.003$) are also found. 
Dealing with the real object ($M=4.00$) is statistically greater than belongings of the virtual object ($M=3.60$). Participants feel more in belongings when they have controllability ($M=5.11$) than when they do not ($M=2.50$). When the partner has controllability ($M=3.59$), the perceived belongings is lower than when the partner lacks controllability ($M=4.02$).
% There are no interaction effects. The significant main effects are found for Cube Tangibility ($p\textless.001$, $F(1, 27)=15.8$, $eta_p2=.369$) and Controllability ($p\textless.001$, $F(3, 81)=77.0$, $eta_p2=.740$). 


\textbf{Sense of control:} We find an interaction effect between PTC and PNC ($p=.011$).
% We find an interaction effect between PTC and PNC ($p=.011$,  $F(1, 27)=7.38$, ${\eta_p}^2=.215$).
The simple effects of PTC is discovered in both cases when the partner have and do not controllability, showing ($p\textless.001$, $F(1, 27)=133$, ${\eta_p}^2=831$) and ($p\textless.001$, $F(1, 27)=305$,  ${\eta_p}^2=.919$) respectively. In the former case, when the participants have controllability ($M=5.45$), it shows greater sense of control than when they do not have controllability ($M=2.05$). The latter case also shows the similar results. The greater sense of control is found when the participants have controllability ($M=6.15$),  than when they do not have ($M=2.10$). 
% A simple effect of PNC when the participants have controllability is reported ($p\textless.001$).%,  $F(1, 27)=14.2$, ${\eta_p}^2=.345$). 
In our further analysis, it is significantly higher when only the participants have controllability ($M=6.15$) than when both have ($M=5.45$).

We also find the main effects of OP ($p=.041$), PTC ($p\textless.001$), and PNC ($p=.008$).
% We also find the main effects of OP ($p=.041$,  $F(1, 27)=4.61$, ${\eta_p}^2=.146$), PTC ($p\textless.001$,  $F(1, 27)=244$, ${\eta_p}^2=.900$), and PNC ($p=.008$,  $F(1, 27)=8.14$, ${\eta_p}^2=.232$).
The sense of control over the real cube ($M=4.04$) is statistically greater than the sense over the virtual cube ($M=3.82$). When the participants have controllability ($M=5.80$), they feel more in control than when they do not ($M=2.06$). When the partner has controllability ($M=3.73$), a weaker sense of control is reported than the partner lacks controllability ($M=4.13$).

% While no interaction effect is found, the significant main effects of Cube Tangibility ($p=.041$,  $F(1, 27)=4.62$, ${\eta_p}^2=.146$) and Controllability ($p\textless.001$,  $F(3, 81)=159$, ${\eta_p}^2=.855$) are found. 


\textbf{Sense of bond:} An interaction effect between PTC and PNC ($p\textless.001$) is found. 
% An interaction effect between PTC and PNC ($p\textless.001$,  $F(1, 27)=18.1$, ${\eta_p}^2=.401$) is found. 
We only find a simple effect of PNC ($p\textless.001$).%,  $F(1, 27)=17.1$, ${\eta_p}^2=.388$). 
When only the participants have controllability ($M=5.07$), the sense of bond scores is significantly higher than when both have ($M=4.39$).
% No interaction effects between the independent variables are found. 

Significant main effects of OP ($p=.008$), PTC ($p\textless.001$), and PNC ($p=.021$) are reported. 
% Significant main effects of OP ($p=.008$,  $F(1, 27)=8.08$, ${\eta_p}^2=.230$), PTC ($p\textless.001$,  $F(1, 27)=124$, ${\eta_p}^2=.821$), and PNC ($p=.021$,  $F(1, 27)=6.02$, ${\eta_p}^2=.182$) are reported.
In terms of OP, the real cube case ($M=3.54$) has a statistically higher sense of bond than the virtual cube ($M=3.26$). When participants have controllability ($M=4.73$), they report a stronger sense of bond than when they do not ($M=2.07$). However, a weaker bond is reported when the partner has controllability ($M=3.25$) compared to when they do not have controllability ($M=3.55$).

% Significant main effects of Cube Tangibility ($p=.008$,  $F(1, 27)=8.08$, ${\eta_p}^2=.230$) and Controllability ($p\textless.001$,  $F(3, 81)=91.3$, ${\eta_p}^2=.772$) are reported. 

\textbf{Sense of Separatiton:} 
We find an interaction effect between OP and PNC ($p\textless.001$). 
% We find an interaction effect between OP and PNC ($p\textless.001$,  $F(1, 27)=13.7$, ${\eta_p}^2=.337$). 
Only a simple effect of PNC with the virtual cube ($p\textless.001$, $F(1, 27)=18.1$, ${\eta_p}^2=.402$) 
is disclosed. When the object is virtual, the partner's controllability over the object ($M=4.88$) raises the sense of separation from the object more than if the partner has no controllability over the object ($M=4.34$). 

% We find an interaction effect between Cube Tangibility and Controllability ($p=.002$,  $F(3, 81)=6.514$, ${\eta_p}^2=.194$). We find a simple effect of Controllability with Cube Tangibility at physical ($p\textless.001$,  $F(3, 81)=16.2$, ${\eta_p}^2=.375$) and virtual ($p\textless.001$, $F(3, 81)=28.0$, ${\eta_p}^2=.510$). When the object is physical, controllability on the participants ($M$=3.73) has the significantly lower sense of separate to the object than the cases of controllability on the partner ($M$=5.07, $p$=.005) and neither ($M$=5.13, $p$=.005). We also find the case when both have controllability of the object ($M$=3.46), the participants felt the significantly lower sense to the object than the cases of controllability on the partner ($p$\textless.001) and neither ($p$\textless.001). We find no differences in the other cases. When the object is virtual, controllability on the participants ($M$=3.28) has the significantly lower sense of separate to the object than all the cases (Both: $M$=4.08, $p$=.001, Neither: $M$=5.411 $p$\textless.001, and Partner: $M$=5.68, $p$\textless.001). When both can control the virtual object, significantly low senses are also discovered compared to the Neither($p$=.008) and Partner ($p$\textless.001) cases. No difference between the Neither and Partner cases ($p$=.654).

Significant main effects of OP ($p=.036$) and PTC ($p\textless.001$) are reported.
% Significant main effects of OP ($p=.036$,  $F(1, 27)=4.88$, ${\eta_p}^2=.153$) and PTC ($p\textless.001$,  $F(1, 27)=32.1$, ${\eta_p}^2=.543$) are reported.
The virtual cube object ($M=4.62$) strengthens the sense of separation more than the real cube ($M=4.35$). In addition, the sense of separation is intensified when the participants could not control the object ($M=5.32$) compared to when they could ($M=3.64$).

% significant effects of Cube Tangibility ($p=.036$,  $F(1, 27)=4.88$, ${\eta_p}^2=.153$) and Controllability ($p\textless.001$,  $F(3, 81)=26.1$, ${\eta_p}^2=.492$).


\textbf{Sense of coexistence - object:} There is a significant interaction effect between OP and PP ($p=.030$). 
% Firstly, we find an interaction effect between OP and PP ($p=.030$,  $F(1, 27)=5.28$, ${\eta_p}^2=.163$). 
A simple effect of PP when the object is physical ($p=.007$)%,  $F(1, 27)=8.41$, ${\eta_p}^2=.237$) 
is apparent, but not when the object is virtual ($p=.732$). Interestingly, when the partner is the real human ($M=6.44$) rather than the virtual ($M=5.92$), a significantly higher sense of object coexistence is reported. 
Next, there is another interaction effect between OP and PTC ($p=.027$) is disclosed. 
% Next, an interaction effect between OP and PTC ($p=.027$,  $F(1, 27)=5.45$, ${\eta_p}^2=.168$) is disclosed. 
Simple effects of PTC are discovered when the OP is real ($p\textless.001$)%,  $F(1, 27)=16.6$, ${\eta_p}^2=.381$) 
and virtual cubes ($p\textless.001$)
%,  $F(1, 27)=26.1$, ${\eta_p}^2=.492$), 
respectively. The results reveal that when the participants have control over the real object ($M=6.55$), they have a higher feeling of coexisting with it than when they do not ($M=5.81$). When the object is virtual, similar results are reported. The participants also have a higher feeling of coexisting with the virtual object when they have control over the object ($M=4.63$) than when they do not ($M=3.40$).

The main effects of OP ($p\textless.001$) and PTC ($p\textless.001$) are found.
% The main effects of OP ($p\textless.001$, $F(1, 27)=.76.9$, $eta_p2=.740$) and PTC ($p\textless.001$, $F(1, 27)=28.4$, $eta_p2=.512$) are found.
It is found that the real cube ($M=6.18$) makes the participants feel a stronger sense of coexistence than the virtual cube ($M=4.01$). The participants also have a stronger sense of coexistence with the object when they can control the object ($M=5.59$) than when they cannot ($M=4.60$).

% We additionally find the main effects of Cube Tangibility ($p\textless.001$, $F(1, 27)=.76.9$, $eta_p2=.740$) and Controllability ($p\textless$, $F(3, 81)=17.9$, $eta_p2=.398$). 

\textbf{Sense of coexistence - partner:} PTC and PNC have a significant interaction effect ($p=.047$).
% PTC and PNC have a significant interaction effect ($p=.047$, $F(1, 27)=4.34$, $eta_p2=.139$).
When the participants have controllability, a simple impact of PNC is found ($p=.002$).%, $F(1, 27)=11.7$, $eta_p2=.303$). 
Interestingly, when the partner could control the object ($M=5.52$), the sense of coexistence is improved much higher than when the partner could not  ($M=5.14$).

We find two main effects of PP ($p\textless.001$) and PNC ($p=.016$). 
% We find two main effects of PP ($p\textless.001$, $F(1, 27)=84.6$, $eta_p2=.758$) and PNC ($p=.016$, $F(1, 27)=6.59$, $eta_p2=.196$).
Understandably, the real partner ($M=6.68$) has a greater sense of coexistence than the virtual human ($M=6.68$). Furthermore, when the partners have control over the things ($M=5.34$) and when they do not ($M=5.10$), the participants perceive a better coexistence with the partners for the former case. 

% The significant main effects of Partner Tangibility ($p\textless.001$, $F(1, 27)=84.7$, $eta_p2=.758$) and Controllability ($p=.005$, $F(3, 81)=.4.54$, $eta_p2=.144$) are found. No interaction effects are reported.



\subsubsection{Regression Results on Ownership}

We found a statistically significant relationship between the sense of control (p=.001), sense of separate  (p\textless.001), and partner presence (p=.010) with ownership, but not between the sense of belonging  (p=.293) and cube presence (p=.771) and ownership. Its results are reported in Fig.~\ref{fig_regression_result}.

To quantify the strength of the association between the sense of control, sense of separateness, and partner presence with ownership, we report the odds ratio (OR) for each variable. OR is defined as the likelihood of an outcome occurring given a specific exposure, as opposed to the likelihood of the outcome occurring in the absence of that exposure. The odds of ownership increased by 23\% (95\% CI [-.16,.81]) for the sense of control and decreased by 31\% (95\% CI [-.44, -.16]) and 27\% (95\% CI [-.43, -.07]) for the sense of separation and partner presence, respectively.





==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

